Generating Features with Increased Crop-related Diversity for Few-Shot Object Detection

Two-stage object detectors generate object proposals and classify them to detect objects in images. These proposals often do not contain the objects perfectly but overlap with them in many possible ways, exhibiting great variability in the difficulty levels of the proposals. Training a robust classifier against this crop-related variability requires abundant training data, which is not available in few-shot settings. To mitigate this issue, we propose a novel variational autoencoder (VAE) based data generation model, which is capable of generating data with increased crop-related diversity. The main idea is to transform the latent space such latent codes with different norms represent different crop-related variations. This allows us to generate features with increased crop-related diversity in difficulty levels by simply varying the latent norm. In particular, each latent code is rescaled such that its norm linearly correlates with the IoU score of the input crop w.r.t. the ground-truth box. Here the IoU score is a proxy that represents the difficulty level of the crop. We train this VAE model on base classes conditioned on the semantic code of each class and then use the trained model to generate features for novel classes. In our experiments our generated features consistently improve state-of-the-art few-shot object detection methods on the PASCAL VOC and MS COCO datasets.

==> anlysis_1shot.tex <==

\begin{figure}[t]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=0.4\linewidth]{latex/figs/teaser.png}
\end{center}
\caption{
% 
\textbf{One-shot classification accuracy with different support image-- }
FSL methods heavily depend on how representative the support samples are. The figure shows the one-shot accuracy of the Meta-Baseline method and our method when using 5 different support images whose $L_{2}$ distances to the mean feature of the class "X" ranged from 0.5 to 0.7. The accuracy fluctuates from 72\% to 32\% for Meta-Baseline when using different support images.
}
\label{fig:one-shot}
\end{figure}


\section{One-shot classification accuracy with different support image}
\label{sec:one-shot}


\begin{figure}[t]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=0.5\linewidth]{latex/figs/one-shot.png}
\end{center}
\caption{
% 
\textbf{One-shot classification accuracy with different support image-- }
FSL methods heavily depend on how representative the support samples are. The figure shows the one-shot accuracy of the Meta-Baseline method and our method when using 5 different support images whose $L_{2}$ distances to the mean feature of the class "X" ranged from 0.5 to 0.7. The accuracy fluctuates from 72\% to 32\% for Meta-Baseline when using different support images.
}
\label{fig:one-shot}
\end{figure}

==> exp.tex <==
\subsection{Mapping Function Analysis}
We use a simple pre-defined linear function $g(x) = w\times x + b$ to map from an IoU score $x$ to the new norm of a latent code. Here we only consider proposals with IoU scores ranging from 0.5 to 1. When using proposals whose IoU scores are lower than 0.5, we observe significant performance drops. A potential reason is that the proposals with little overlap with the objects contain mostly background pixels, and thus can be noisy training signals for the VAE model.
The coefficients of the linear function can be inferred by defining the value range of the rescaled latent norm. We conduct experiments with different ranges and the results are shown in Table \ref{tab:g_function}. Note that here $\sqrt{512}$ is a scaling constant that corresponds to the number of dimension ($N = 512$) of the latent space. 
As can be seen from the table, we observe better performance when the IoU score inversely correlates the latent norm. In this case, a proposal with low IoU score has a higher latent norm and is placed further away from the origin. A possible reason is that features of hard instances often exhibit higher variance. Thus, it is more optimal to use latent codes with larger norms to represent them \cite{Meng2021MagFaceAU}.
\label{sec:g}
\begin{table}[!h] 
  \centering
\resizebox{0.45\textwidth}{!}{%
  \begin{tabular}{c|ccc}
    \toprule
      & $g$(1) & $g$(0.5) & AP50 \\
    \midrule 
     \multirow{3}{*}{Inverse Correlation} & {1$\times\sqrt{512}$} & {2$\times\sqrt{512}$} & {61.6}  \\
     & {1$\times\sqrt{512}$} & {5$\times\sqrt{512}$} & \textbf{62.1}  \\
      & {1$\times\sqrt{512}$} & {10$\times\sqrt{512}$} & {61.8}  \\
    \midrule 
     \multirow{3}{*}{Correlation} & {2$\times\sqrt{512}$} & {1$\times\sqrt{512}$} & {60.6} \\
     & {5$\times\sqrt{512}$} & {1$\times\sqrt{512}$} & {61.3}  \\
      & {10$\times\sqrt{512}$} & {1$\times\sqrt{512}$} & {60.6}  \\
    \bottomrule
  \end{tabular}}
  \\ \vspace{6pt}
  \caption{\textbf{Performance with different configurations of the mapping function}. We conduct experiments using different coefficients for function $g(\cdot)$, which defines the value range of the new norm of the latent code.   %CLIP \citep{Radford2021LearningTV_CLIP} is trained with 400M pairs (image and its text title) collected from the web while Word2Vec \citep{Mikolov2013EfficientEO} is trained with only text data.
  %Best performance  in bold.
    }\label{tab:g_function}%
  \vspace{-10pt}
\end{table}


 
 \subsection{Effectiveness of Patch Selection}
 Our strategy for zero-shot counting is to select patches across the query image and use them as exemplars for counting. The patches are selected via a generated class prototype and an error predictor. An alternative way is to use the generated prototype to do correlation matching directly instead of selecting patches from the input image. In this section, we compare the performance of these two strategies and show the advantage of our proposed one. Specifically, we use the prototype computed in Eq. \ref{eq:prototype} to do correlation matching with the features of input images to get the similarity map, which will be then inputted to the counter to get the density map and final count. The VAE used to generate the prototype in our main experiments is trained on MS-COCO detection set. We train another VAE using FSC-147 training set and report the performance with both VAEs in Table \ref{tab:patch_selection}. As can be seen, our proposed patch selection method achieves better results. Directly using the generated prototype to do correlation matching provides a simple solution for zero-shot counting. However, it is not optimal since the same prototype is applied for all the objects from different images. These objects typically exhibit large variation. Our patch selection method, in comparison, select different exemplars dynamically according to the input image. %The selected exemplars are more likely to share fine-grained details with the objects in the image compared with a universal prototype.
\begin{table*}[!h] 
  \centering
\resizebox{0.72\textwidth}{!}{%
  \begin{tabular}{c|c|cccc|cccc}
    \toprule
   \multirow{2}{*}{\parbox{1.5cm}{Patch \\ selection}}& \multirow{2}{*}{\parbox{2cm}{Training data\\for VAE}} & \multicolumn{4}{c|}{Val Set} & \multicolumn{4}{c}{Test Set} \\
    & & MAE & RMSE & NAE & SRE & MAE & RMSE & NAE & SRE \\
    \midrule
    \xmark & MS-COCO & {48.56} & {127.93} & 0.65 & 6.37 & {41.33} & {147.43} & 0.52 & 5.53 \\ 
    \xmark & FSC-147 & {30.51} & {101.39} & 0.41 & 4.66 & {28.03} & {132.34} & 0.37 & 4.42 \\
    \Checkmark & MS-COCO & \textbf{27.00} & \textbf{87.90} & \textbf{0.35} & \textbf{4.29} & \textbf{22.09} & \textbf{115.17} & \textbf{0.34} & \textbf{3.74} \\
    \bottomrule
  \end{tabular}} \\ \vspace{6pt}
  \caption{ {Comparison between our proposed method and directly using the class prototype to do correlation matching.} 
  }\label{tab:patch_selection}%
  \vspace{-10pt}
\end{table*}






==> intro.tex <==
Specifically, to select class-relevant patches, we first use a generative model to obtain a class prototype for the given class in a pre-trained feature space. This class prototype can be viewed as a class center representing the distribution of the features from that class in the feature space.
%
Then given a query image, we randomly sample a number of patches of various sizes and extract the corresponding feature embedding for each patch. Since the pre-trained feature space is highly discriminative, patches whose embeddings are close to each other are likely to contain objects from the same class. Therefore, we select the patches whose embeddings are the nearest neighbors of the class prototype as the class-relevant patches. 
%

After obtaining class-relevant patches, we use our introduced model to select the most suitable patches for counting.          
%To do this, we introduce a counting error regressor that can predict the counting error produced by an arbitrary image patch. 
%when being used as the counting exemplar. 
%To train this error regressor, given a query image and an arbitrary patch cropped from this image, we first use a pre-trained object counter to compute the counting error using this patch as the exemplar. 
To train this model, given a query image and an arbitrary patch cropped from this image, we first use a pre-trained exemplar-based counting model to obtain the intermediate feature maps and calculate the corresponding counting error. The counting error can be considered as a quantitative measurement to measure how suitable the patch is as a counting exemplar, {i.e.}, smaller counting error indicates a more suitable image patch for counting.
%
Our introduced model then takes the feature maps as input and tries to predict the counting error. After this counting error predictor is trained, we can apply it on all the candidate patches to get the error of each candidate and select those with the smallest errors as the final counting exemplars. 


exemplar-free class-agnostic counting has been recently proposed as a useful task. Although exemplar-based class-agnostic counting has achieved tremendous progress in recent years \cite{Lu2018CAC,Ranjan2021LearningTC, Yang2021ClassagnosticFO,Shi2022SimiCounting,Gong2022ClassIntra,Nguyen2022fsoc,Liu2022CounTRTG}, exemplar-free object counting is a far less explored problem. The only previous work on counting without exemplar,

In this paper, we go one step further by introducing the task of zero-shot object counting (ZSC), which focuses on counting instances of a specific class given only the class name.

==> latex/backup.tex <==
Recent years have witnessed great progress in class-agnostic object counting (CAC), which aims to count objects of arbitrary categories in a given query image. A human user is required in the process to specify the object category of interest by providing a few exemplars. However, for many real applications such as medical and manufacturing, providing exemplars for each query image is time-consuming and needs expert supervision. The labeling effort of human-annotated exemplars hinders the applicability of performing object counting for realistic large-scale datasets.

To this end, we introduce the task of zero-shot counting (ZSC), which aims to count instances of arbitrary class without any annotated exemplars. 
Exemplars are essentially some human annotated patches within the input image that are suitable for counting, \textit{i.e}, containing the object of interests. 
%
To obtain the exemplars for counting, we introduce a regressor module that can measure how suitable of a patch is for counting and use this regressor to select the suitable ones among all the patches.
%
Specifically, given a pre-trained counting model and an input image for counting, we first randomly sample patches of various sizes across the image. Each of the sampled patch is then used as an exemplar for counting and we can obtain the corresponding counting error. 
%
The smaller the counting error, the more suitable the patch is for counting. 
%
We do this for all the images in the training set, which provides us thousands of pairs of patch and its corresponding counting error. We then optimize the regressor to output the counting error for each input patch. 
%
After the regressor is trained, given an input query image, we randomly sample patches across the image and feed them into the trained regressor. The patches with small predicted counting errors will be selected as optimal patches and used as exemplars for counting. 

The main challenge for zero-shot counting is that we do not have access to exemplars in the counting process. 

Generally, exemplar-based CAC methods work in an extract-and-match pipeline. They first extract visual features from exemplars and match these features with those of query images. Similarity maps are then used as intermediate representations to infer object counts. In zero-shot counting where we do not have access to exemplars in the counting process, it is infeasible to extract visual features from exemplars and do correlation matching to get the similarity map for counting. Inspired by feature-generation based methods for other zero-shot learning tasks, \textit{i.e}, zero-shot image classification, one possible solution is to use generative models to hallucinate visual features based on the given class name and use the generated features to do similarity matching. This generative model is trained with sufficient data conditioned on the corresponding class name. After the generative model is trained, we use it to generate 

However, objects from different images typically exhibit great variations in terms of image style such as brightness, background lightness, etc. The style of the templates for counting are expected to be consistent with that of the query image.  
%for different query images, the templates are supposed to be different according to the style of the image, \textit{i.e}, brightness, contrast, and background lightness. 
For exemplar-based counting methods where the exemplars are the crops from the input image, the style of the templates and the query image are intrinsically the same. However, in our case where the template features are generated from a generative model, it is non-trivial to enforce the style of the templates to be consistent with that of the query image. 



There are two main challenges for zero-shot object counting in the wild. First, there is no access to any human-annotated exemplars in the counting process. These exemplars typically contain the objects of interests and can serve as templates to obtain the similarity map via correlation matching with the query image. Secondly, there often exists non-relevant objects for query images in the wild that can potentially confuse the object counter. 

The main challenge for zero-shot object counting is that there is no access to exemplars in the counting process. These exemplars typically serve as counting templates to match with the features of query images. Similarity maps are then used as intermediate representations to infer object counts. In zero-shot counting where we do not have access to exemplars, it is infeasible to obtain class templates from exemplars and do correlation matching to get the similarity maps. Inspired by feature-generation based methods for other zero-shot learning tasks, \textit{i.e}, zero-shot classification, one possible solution is to use generative models to hallucinate visual features based on the given class name and use the generated features as templates to do similarity matching. Despite being simple and intuitive, a major drawback of this method is that the same matching templates are used for all the input query images of that class.
%Applying a single template on different query images for obtaining similarity maps is not optimal. 
This is not optimal since objects from different images can be greatly different in terms of shapes, scales, illuminations, and backgrounds.
%
In comparison, exemplar-based counting methods use separate templates for each input query image.
%obtain the matching template via  human-annotated patches which are part of the query image. 
%
These patches are more likely to share fine-grained similarities with the objects for counting since they are from the same image.

To this end, instead of directly using the generated features as templates, we use them to select patches across the query image which will then serve as exemplars for counting. Specifically, given an arbitrary class name, we first use the generative model to obtain a visual feature prototype for this class. Then we randomly sample a number of patches across the query image and extract their corresponding visual features. Based on the euclidean distance between the extracted features and the class prototype, we can select the patches with close distance to the prototype. These patches possibly contain the object of interests and can be used as exemplars for counting. 

\begin{mycomment}

\end{mycomment}

Exemplar-based methods have shown tremendous successes in CAC. These methods extract visual templates from exemplars and correlate them with the features of input images to obtain a similarity map for counting. %In zero-shot counting where we do not have access to exemplars in the counting process, it is infeasible to obtain class templates from exemplars and do correlation matching to get the similarity maps.
In our case where no exemplar is provided, an alternative solution is to use a generative model to
%Inspired by feature-generation based methods for other zero-shot learning tasks, \textit{i.e}, zero-shot classification, one possible solution is to use generative models to 
hallucinate visual features based on the given class name and use the generated features as templates to do similarity matching. Here the same class template would be used for all input images for counting that specific class. 
However, it is not optimal to use a common class-specific template for all images since the object appearances can be wildly different in terms of shapes, scales, illuminations, and backgrounds.
%
In comparison, exemplar-based counting methods use separate templates for each input query image.
%obtain the matching template via  human-annotated patches which are part of the query image. 
%
These patches are more likely to share fine-grained similarities with the objects for counting since they are from the same image.


To this end, rather than directly use the generated features as templates, we propose to use them to select image patches and use them as templates. Specifically, given an arbitrary class name, we first use the generative model to obtain a visual feature prototype for this class. Then we randomly sample a number of patches across the query image and extract their corresponding visual features. Based on the euclidean distance between the extracted features and the class prototype, we can select the patches with close distance to the prototype. These patches possibly contain the object of interests and can be used as exemplars for counting.  

The above strategy enables us to obtain class-relevant templates dynamically according to the input query image without relying on any human-annotated exemplars. However, it is not guaranteed that all patches containing object of interests are optimal exemplars for counting. For example, some selected patches might contain only part of the object; some patches are not representative for other objects in the same image. To this end, we equip our zero-shot counter with a patch selection model to further identify the most suitable patch for counting. The assumption here is that we can measure how suitable a patch is for counting by the counting error produced by the patch when being used as the matching template. Based on this assumption, we train the patch selection model to predict the counting error given an arbitrary patch from the query image. After the patch selection model is trained, we can select the patches with smallest counting errors and use them as the templates for counting.



Specifically, we guide the VAE model to generate representative samples by selecting only representative data from the base classes for training it. In essence, our VAE model is trained to model the data distribution of the training set. As the training set contains only representative data, the trained VAE model outputs samples that are also representative. Specifically, to select those representative features, we first assume that the feature vectors of each class follow a multivariate Gaussian distribution and estimate this distribution for each base class. Based on these distributions, we compute the probability of each sample belonging to its corresponding category to measure the representativeness for the sample. We filter out the non-representative samples and train the VAE using only representative samples. Interestingly, we show that the representativeness of the training set highly corresponds to the accuracy of the few-shot classifier. We obtain the highest accuracy when training the VAE with the most representative samples. In this case, we only use a small percentage of the whole training set, e.g., 10\% for the case of \textit{mini}Imagenet dataset, to obtain the best results. Our analyses show that 
this approach consistently improves the FSL classification performance by $1\sim2\%$ across all benchmarks for three different baselines\cite{metabaseline,protonet,Liu2020AnEO}.

To this end, we introduce the task of zero-shot counting (ZSC), which aims to count instances of arbitrary class without any human-annotated exemplars. Given a query image, our visual counter only requires the semantic knowledge of the object of interest without any human user in the loop. 
This will be very crucial for building fully automated systems in various applications in wildlife monitoring, healthcare and visual anomaly detection. For example, this visual counter can be used to alert environmentalists when a herd of animals with significant size pass by an area monitored by a wildlife camera. Another example is to use this visual counter to monitor for critical health conditions when any certain type of cells outgrows the other types. 

\begin{table}[!h] 
  \centering
\resizebox{0.48\textwidth}{!}{%
  \begin{tabular}{l|c|cc|cc}
    \toprule
   \multirow{2}{*}{Method} & \multirow{2}{*}{Exemplars} & \multicolumn{2}{c|}{Val Set} & \multicolumn{2}{c}{Test Set} \\
    & & MAE & RMSE & MAE & RMSE \\
    \midrule
    \multirow{2}{*}{GMN} & GT & {29.66} & {89.81} & {26.52} & {124.57}  \\
    & RPN & {39.02} & {106.06} & {37.86} & {141.39}  \\
    \midrule
    %\multirow{2}{*} {FamNet} & GT & {24.32} & {70.94} & {22.56} & {101.54} \\
    % & RPN & {48.62} & {120.77} & {53.82} & {155.38}  \\
    %\midrule
    \multirow{2}{*}{FamNet+} & GT & {23.75} & {69.07} & {22.08} & {99.54} \\
     & RPN & {42.85} & {121.59} & {42.70} & {146.08}  \\
     \midrule
     \multirow{2}{*}{BMNet} & GT & {19.06} & {67.95} & {16.71} & {103.31} \\
     & RPN & {32.19} & {99.21} & {37.22} & {143.13}  \\
     \midrule
    \multirow{2}{*} {BMNet+} & GT & {15.74} & {58.53} & {14.62} & {91.83} \\
     & RPN & {35.10} & {106.07} & {34.52} & {132.64}  \\
    \midrule
    %{FamNet} & {32.15} & {98.75} & {32.27} & {131.46} \\
    %{BMNet} & & {34.09} & {105.05} & {31.27} & {124.85} \\
    %{BMNet+} & & {35.15} & {106.07} & {34.52} & {132.64} \\
    %{BMNet+} & {23.01} & {72.61} & {22.43} & {128.12} \\
    {RepRPN-Counter} \cite{Ranjan2022Exemplar} & - & {29.24} & {98.11} & {26.66} & {129.11} \\
    \midrule
    \multirow{2}{*}{Ours (Base)} & GT & {18.55} & {61.12} & {20.68} & {109.14} \\
     & Ours & \textbf{27.00} & \textbf{87.90} & \textbf{22.09} & \textbf{115.17} \\
    \bottomrule
  \end{tabular}} \\ \vspace{6pt}
  \caption{ \textbf{Comparison between models trained with different groups of generated features}. The model trained with ``Low-IoU'' features has better nAP50 scores while the ``High-IoU'' model has better nAP75 scores.
  %Features corresponding to different IoUs improve the performance differently in terms of nAP50 and nAP75.
  }\label{tab:test_val}%
  \vspace{-10pt}
\end{table}


\begin{table}[!h] 
  \centering
\resizebox{0.48\textwidth}{!}{%
  \begin{tabular}{l|cc|cc}
    \toprule
   \multirow{2}{*}{Method} & \multicolumn{2}{c|}{Val Set} & \multicolumn{2}{c}{Test Set} \\
    & MAE & RMSE & MAE & RMSE \\
    \midrule
    {GMN} & {39.02} & {106.06} & {37.86} & {141.39}  \\
    %{MAML} & {32.44} & {101.08} & {31.47} & {129.31} \\ 
    {FamNet} & {48.62} & {120.77} & {53.82} & {155.38} \\
    {FamNet+} & {39.52} & {116.08} & {39.38} & {143.51} \\
    %{FamNet} & {32.15} & {98.75} & {32.27} & {131.46} \\
    {BMNet} & {34.09} & {105.05} & {31.27} & {124.85} \\
    {BMNet+} & {35.15} & {106.07} & {34.52} & {132.64} \\
    %{BMNet+} & {23.01} & {72.61} & {22.43} & {128.12} \\
    {RepRPN-Counter} & {29.24} & {98.11} & {26.66} & {129.11} \\
    {Ours} & \textbf{27.00} & \textbf{87.90} & \textbf{22.09} & \textbf{115.17} \\
    \bottomrule
  \end{tabular}} \\ \vspace{6pt}
  \caption{ \textbf{Comparison between models trained with different groups of generated features}. The model trained with ``Low-IoU'' features has better nAP50 scores while the ``High-IoU'' model has better nAP75 scores.
  %Features corresponding to different IoUs improve the performance differently in terms of nAP50 and nAP75.
  }\label{tab:test_val}%
  \vspace{-10pt}
\end{table}

\begin{table}[!h] 
  \centering
\resizebox{0.3\textwidth}{!}{%
  \begin{tabular}{l|cc|cc}
    \toprule
   \multirow{2}{*}{n} & \multicolumn{2}{c|}{Val Set} & \multicolumn{2}{c}{Test Set} \\
    & MAE & RMSE & MAE & RMSE \\
    \midrule
    {1} & {39.02} & {106.06} & {37.86} & {141.39}  \\
    {3} & {32.44} & {101.08} & {31.47} & {129.31} \\ 
    {5} & \textbf{27.54} & \textbf{87.95} & \textbf{22.93} & \textbf{127.87} \\
    \bottomrule
  \end{tabular}} \\ \vspace{6pt}
  \caption{ \textbf{Comparison between models trained with different groups of generated features}. The model trained with ``Low-IoU'' features has better nAP50 scores while the ``High-IoU'' model has better nAP75 scores.
  %Features corresponding to different IoUs improve the performance differently in terms of nAP50 and nAP75.
  }\label{tab:number}%
  \vspace{-10pt}
\end{table}

==> latex/bak.tex <==

\section{Overview}
%In this document, we provide additional experiments and analyses. In particular:
\begin{itemize}
    \item Section \ref{sec:vae_underfit} shows the few-shot performance of our method where we use a deeper network architecture for the decoder of our VAE model. 
     \item Section \ref{sec:visualization} provides visualization of representative and non-representative samples selected via our method for some classes of the \textit{tiered}ImageNet dataset\cite{Ren2018MetaLearningFS_tieredImagenet}.
    \item Section \ref{sec:distribution_analysis} shows the percentages of the selected samples for some base classes via our feature selection method. We show that filtering samples lead to smaller distances between ground truth prototypes and estimated prototypes.
    
    \item Section \ref{sec:one-shot} shows the 1-shot accuracy of our method in comparison with Meta-Baseline\cite{metabaseline} using different support samples. 
    \item Section \ref{sec:zsl}, we provide multiple additional experiments and analyses of our method.
    \item Section \ref{sec:new}, we provide multiple additional experiments and analyses of our method.
\end{itemize}

==> relatedwork.tex <==

Learning from auxiliary 

VAEs have been widely used in Zero-Shot Learning (ZSL) where we assume that no image of novel classes is available during training.  ZSL methods thus rely on an auxiliary modality containing some information of the unseen classes such as textual descriptions [more papers] or attribute vectors \cite{Devise_13} and focuses on learning the relationship between the visual and the auxiliary domains. For example, Frome \etal propose using a semantic embedding space to 

The concept of aligning the semantic embedding space and the visual embedding space has been used in some ZSL methods \cite{Devise_13}. Tsai \etal propose to learn joint embeddings for semantic and visual features in which they align the feature distributions between the two domains.

However, it is not trivial to simply apply them to a few-shot learning setting.   

\cite{Huang2021AGAM}

xx aims to associate pre-trained visual feature
representations to each attributes via 

Adaptive Cross-Modal Few-shot Learning

Generalized Zero- and Few-Shot Learning via Aligned Variational Autoencoders
